WordRobe: Text-Guided Generation of Textured 3D Garments

In this paper, we tackle a new and challenging problem of text-driven generation of 3D garments with high-quality textures. We propose "WordRobe", a novel framework for the generation of unposed & textured 3D garment meshes from user-friendly text prompts. We achieve this by first learning a latent representation of 3D garments using a novel coarse-to-fine training strategy and a loss for latent disentanglement, promoting better latent interpolation. Subsequently, we align the garment latent space to the CLIP embedding space in a weakly supervised manner, enabling text-driven 3D garment generation and editing. For appearance modeling, we leverage the zero-shot generation capability of ControlNet to synthesize view-consistent texture maps in a single feed-forward inference step, thereby drastically decreasing the generation time as compared to existing methods. We demonstrate superior performance over current SOTAs for learning 3D garment latent space, garment interpolation, and text-driven texture synthesis, supported by quantitative evaluation and qualitative user study. The unposed 3D garment meshes generated using WordRobe can be directly fed to standard cloth simulation & animation pipelines without any post-processing.

==> sec/2_related_work_short.tex <==
\section{Related Work}
\noindent
\textbf{3D Garment Generation:}
Deep learning-based garment digitization solutions\cite{jiang2020bcnet, zhu2022registering, Srivastava2022xClothET} attempt to address the scalability challenge by extracting 3D garment mesh from images. %However, they often reconstruct sub-optimal geometries that are ill-suited for direct integration into standard graphics pipelines. 
Another line of work takes inspiration from real-world garment creation and proposes both analytical\cite{10.1145/3528223.3530145} \& neural methods\cite{KorostelevaGarmentData} for generating production-ready 3D garments. 
% Modelling 3D garment meshes from 2D sewing patterns is a popular choice, where base panels represented using Bezier curves form different parts of a garment. Manipulating the base panels and stitching them together in different ways, governed by a complex clothing simulation-based process, creates different kinds of garments. However, the manipulation is not fully automated, demanding an interactive feedback, making it tedious for a novice end user. Moreover, the semantic relationship between the panels is not meaningful in 2D space. Only when the 3D garment is created, then local neighborhood relationships and geometric properties arise. 
%Their approach of designing 3D garments from 2D panels (sewing patterns) is a popular choice but generation and manipulation are not fully automated, demanding an interactive input and making the process tedious for a novice end user. 
%Moreover, semantic relationships between panels become meaningful only in the 3D context after a complex physics-based cloth simulation process. Hence, it is logical to develop the methodology for generating garments directly in the 3D space. Various approaches have emerged in this direction, with the majority of them employing 
Some of the recent approaches\cite{corona2021smplicit, deepcloth_su2022} avoid panel-based generation by building upon parametric human body templates (e.g., SMPL\cite{SMPL:2015}) to generate parametric garments. 
%Nevertheless, the garments generated based on SMPL topology tend to be tight-fitted, lack realism and miss key features such as collars, hoods, pleats, etc. 
In the past few years, data-driven neural implicit methods\cite{mescheder2019occupancy, Park_2019_CVPR} have shown significant promise in modeling 3D shapes. 
%DrapeNet\cite{de2023drapenet} demonstrates the capability of MLPs to learn the shape distribution of 3D garments by encoding them in a latent space and decoding them into the Unsigned Distance Function (UDF) representation which is ideal for modeling garments. The latent space enables controllable editing of garments by modifying the latent codes. However, the latent manipulation is defined by explicit annotations which require significant effort in the case of garments of different categories, made of different components. Additionally, it doesn't offer any texture support which is a crucial characteristic of any garment. \textbf{WordRobe} is able to generate high-quality geometry and synthesize high-fidelity textures as well, from a simple text prompt.
\\
\noindent
\textbf{Text-to-3D:} 
%Recent advancements in vision and NLP research \cite{Radford2021LearningTV, rombach2022highresolution, ho2022imagen, poole2022dreamfusion} have enabled generating concepts of any modality (image, video, 3D, etc.) from user-friendly text prompts in natural language. 
Recently, various text-to-3D methods have been proposed \cite{raj2023dreambooth3d, wang2023prolificdreamer, Chen_2023_ICCV, sun2023dreamcraft3d, poole2022dreamfusion,gao2023textdeformer, shen2021deep} which leverage powerful imaginative capabilities of text-to-image (T2I) models \cite{rombach2022highresolution}, combined with popular 3D representations (NeRF\cite{mildenhall2020nerf}, DMTet\cite{shen2021deep}, etc.) to generate 3D assets from the text. For a given prompt, the above methods optimize the 3D generation, which incurs a large computational cost, and becomes infeasible for the task of generating a large number of 3D garments. NeRF based text to 3D models often lead to noisy surface geometry and artefacts within the scene.

%TextDeformer\cite{gao2023textdeformer} deforms a source mesh into the desired mesh given a text prompt, by leveraging differentiable rendering but does not handle the task of generating a mesh from scratch. 
%Fantasia3D\cite{Chen_2023_ICCV} disentangled the learning of geometry and appearance models which enables the generation of high quality surface geometry and surface material. Dreamfusion\cite{poole2022dreamfusion} and Dreambooth3D\cite{raj2023dreambooth3d} optimise a NeRF model under the condition that the rendering at random viewpoints must belong to the text conditioned distribution by utilising Score Distillation Sampling loss. Prolificdreamer\cite{wang2023prolificdreamer} proposed Variational Score Distillation (VSD) which offers greater generalization and diversity over Score Distillation Sampling (SDS), used by earlier methods. 
% The above methods however, fail to maintain global 3D consistency, due to per-view optimisation and as a result often suffer from inconsistent 3D geometry and appearance. For a given prompt, the above methods optimize the 3D object, which incurs a large computational cost, and becomes infeasible for the task of generating a large number of 3D garments. NeRF based text to 3D models often lead to a noisy surface geometry and artefacts within the scene.\\
% \ar{Mention how these relate to wordrobe in a sentance}
%However, the 3D surface quality obtained through these methods is subpar to that obtained via 3D garment reconstruction methods which are trained specifically to model garments. While the overall quality of text-to-3D methods is expected to improve as research progresses, the inherent 3D representations used by these methods have certain limitations in terms of representing 3D garments with open (non-watertight) surfaces and also lack support for editing or manipulation of garments. Moreover, the majority of these methods rely on a multi-view optimization process which is slow and tedious. \textbf{WordRobe} aims to bridge this gap effectively by allowing the generation and manipulation of production-ready 3D garment meshes from simple text prompts in an optimization-free framework. 
\noindent
\textbf{Text-Guided Texture Synthesis:} 
Several text-guided texture synthesis methods have been proposed ~\cite{text2mesh, khalid2022clipmesh, metzer2022latent, chen2023text2tex} which optimize the clip objective between the input text prompt and differentiably rendered multi-view images. Current SOTA method in text-driven texture synthesis, Text2Tex\cite{chen2023text2tex} utilizes a depth-aware image in-painting diffusion model to progressively fill in texture on a mesh conditioned on a text prompt.
%Text2Mesh\cite{text2mesh} optimizes texture and geometry guided by CLIP objective. CLIPMesh\cite{khalid2022clipmesh} is another CLIP based method which deforms a sphere to generate geometry and optimizes surface color given a text prompt. Latent-Paint\cite{metzer2022latent} generates texture over the UV texture map, by applying the texture to mesh, and then differentiably rendering and optimising over the rendered feature image. The latent texture is passed through the Stable Diffusion decoder once at the end of optimization.
% In particular, Text2Tex\cite{chen2023text2tex} utilizes a depth-aware image in-painting diffusion model to progressively fill in texture on a mesh conditioned on a text prompt. 
%A generation mask is used to guide the model which areas of the mesh remain to be textured. An automatic sequence generation scheme is utilized to determine the next view for depth conditioned in-painting.
%The progressive nature of texture infilling makes this method relatively time consuming. The resultant texture map may also have view inconsistencies because denoising steps in two different views might lead to two slightly different texture images, producing inconsistency. In contrast, WordRobe proposes an optimization free texture generation framework that generates view consistent textures without artifacts.

==> sec/3_background.tex <==
\section{Background}
\textbf{Mesh-UDF:}\\
\\
\noindent
\textbf{CLIP:}\\
\\
\noindent
\textbf{ControlNet:}
